MS-RAFT-3D: A Multi-Scale Architecture for Recurrent Image-Based Scene Flow

Although multi-scale concepts have recently proven useful for recurrent network architectures in the field of optical flow and stereo, they have not been considered for image-based scene flow so far. Hence, based on a single-scale recurrent scene flow backbone, we develop a multi-scale approach that generalizes successful hierarchical ideas from optical flow to image-based scene flow. By considering suitable concepts for the feature and the context encoder, the overall coarse-to-fine framework and the training loss, we succeed to design a scene flow approach that outperforms the current state of the art on KITTI and Spring by 8.7%(3.89 vs. 4.26) and 65.8% (9.13 vs. 26.71), respectively. Our code is available at https://github.com/cv-stuttgart/MS-RAFT-3D.

==> content/related_work.tex <==
% Scene flow estimation is important. What did others do? Why did we do what we did? How does it differ from others? Results. Contributions. Organization.


% Scene flow: 3D motion estimation from RGB-D or stereo image sequences
% Applications: robotics and automotive (collision avoidance, path planning), virtual and augmented reality (markerless motion capture), action recognition and intention prediction
% Base methods:
%  - RAFT-3D: RAFT-based (encoder, cost volume, iterative refinement with RNN), RGB-D based - dedicated network for stereo to RGB-D, soft grouping of rigid moving objects, predict dense field of SE(3) transformations
%  - MS-RAFT: coarse-to-fine extension of RAFT, initialize flow estimation at finer resolution with coarse estimation
% Motivation:
%  - RAFT-3Ds flow refinement only at a resolution of 1/8 -> can miss fine details
%  - MS-RAFT shows effectiveness of multi-scale for related architectures
%  - Multi-scale allows a finer final resolution by initializing prediction with coarser resolutions
% Multi-scale:
%  - Variational methods: avoid local minima and enable estimation of large motion improving accuracy and robustness
%  - In our context: Estimate large motions with local search, estimation at higher resolution (less computational cost than only using the finest scale?)
% Contributions:
%  - Build a multi-scale scene flow method based on RAFT-3D
%  - Multi-scale feature extraction?
%  - Coarse-to-fine initialization of finer scales by upsampling SE(3) scene flow prediction and rigid motion embeddings 
%  - Good performance/improvment on KITTI and Spring
% Related Work:
%  - RAFT: RAFT-3D and MS-RAFT both RAFT-based using similar components: feature & context encoder, 4D hierarchical cost volume, iterative flow refinement with RNN
%  - MS-RAFT/MS-RAFT+/CCMR: multi-scale extension to RAFT with U-Net-style encoder and flow refinement at multiple resolutions with coarse-to-fine initialization
%  - RAFT-3D: RAFT-based scene flow architecture that represents the scene flow prediction as SE(3) field and softly groups rigid moving objects together
%  - Multi-scale used in variational scene flow and optical flow
%  - Multi-scale in deep learning based scene flow: PWOC-3D and SENSE (both PWC-Net based)
%  - Segmentation prominent in recent scene flow publications (RigidMask+ISF, SF2SE3, Deep rigid instance scene flow)
%  - Other scene flow methods:
%     - CamLiFlow/CamLiRAFT: Image + LiDAR point cloud
%     - M-FUSE: Multi-frame fusion based on RAFT-3D
%     - RigidMask+ISF: Segment rigidly moving objects using depth and optical flow estimations. Predict scene flow by the inferred motion of each object
%     - SF2SE3: SE(3) estimation using depth and optical flow estimations. Cluster pixels with similar SE(3) transformations
%     - RAFT-3D
%     - PWOC-3D and SENSE: PWC-Net based multi-scale scene flow methods
%  - Stereo (GA-Net and CroCo-Stereo, RAFT-stereo)?


\noindent \textbf{Stereo and Optical Flow} For the related (sub-)tasks of stereo and optical flow estimation, %there are the approaches of 
Lipson {\em et al.}~\cite{Lipson2021_RAFTStereo}, Li {\em et al.}~\cite{Li2022_CREStereo} and Jahedi {\em et al.}~\cite{MS-RAFT+,CCMR} 
%that 
combine recurrent and multi-scale ideas within a single estimation framework. %The latter ones serve as inspiration for our work.
Moreover, %there are the methods of 
Xu {\em et al.}~\cite{Xu2023_Unifying} and Pan {\em et al.}~\cite{Pan2024_JointRAFTStereoRAFT} %that
seek to improve results for stereo and optical flow by jointly training shared recurrent multi-scale architectures for both tasks (in \cite{Xu2023_Unifying} also with depth). A generalization of these ideas to scene flow, however, has not been investigated in the aforementioned works.

\smallskip

\noindent \textbf{Scene Flow} Regarding 
image-based 
%RGB-D 
scene flow approaches, on the other hand, the underlying models {\em either} employ a multi-scale strategy \cite{PWOC-3D,CamLiFlow} {\em or} they rely on recurrent updates
\cite{RAFT-3D,CamLiRAFT}.
% with the approaches of Liu {\em et al.} \cite{CamLiFlow CamLiRAFT} additionally considering the integration of LiDaR data.
The only exception constitutes the method of Ling {\em et al.}~\cite{ScaleRAFT} that focuses, however, on {\em cross-scale matching} with a corresponding correlation volume and scale look-up operator instead of considering a hierarchical estimation. Moreover, %there is the approach of 
Cheng {\em et al.}~\cite{Cheng2023_MSPointSceneFlow} 
%that also combines
propose to combine multi-scale and recurrent concepts, however, in the context of estimating scene flow from {\em point clouds}.
Finally, it is important to note that all previously mentioned recurrent image-based scene flow approaches \cite{RAFT-3D, CamLiRAFT, ScaleRAFT} work on {\em \textfrac{1}{8} of the original resolution}. Hence, in contrast to our method that operates on \textfrac{1}{2} of the resolution, they require much larger upsampling factors which, in turn, impacts the detailedness of their results.



==> graphics/coarse_to_fine_scheme_horizontal.tex <==
% requires tikz libraries calc, fit, backgrounds

\begin{tikzpicture}[]
    \tikzset{module/.style={draw,thick,rounded corners,inner sep=.15cm,align=center}};
    \tikzset{encoder/.style={fill=white!80!BlueGreen}};
    \tikzset{costvol/.style={fill=white!60!BlueGreen}};
    \tikzset{matching/.style={fill=white!70!Yellow}};
    \tikzset{flow/.style={fill=PineGreen!50!white}};
    \tikzset{supervision/.style={fill=Goldenrod!20!white}}
    \tikzset{upsample_col/.style={fill=red!20!white}}
    \tikzset{arrow/.style={->,very thick,rounded corners}};
    \tikzset{upsample/.style={draw,circle, thick}};

    % Motion embeddings + SE3 field container
    \tikzset{container/.style={draw,thick,rounded corners,inner sep=.15cm,align=center,fill=PineGreen!50!white, minimum width=1.9cm, minimum height=1.6cm}};
    \tikzset{se3_field/.style={draw,thick,rounded corners,inner sep=.15cm,align=center, fill=blue!10, minimum width=1.3cm, minimum height=0.7cm}};
    \tikzset{embedding/.style={draw,thick,rounded corners,inner sep=.15cm,align=center, fill=green!20, minimum width=1.3cm, minimum height=0.7cm}};

    % Iteration loop circled arrows
    \def\circledarrow#1#2#3{
        % Original 3 arrow design.
        %\draw[arrow,#1] (#2) + (30:#3) arc(30:150:#3);
        %\draw[arrow,#1] (#2) + (150:#3) arc(150:270:#3);
        %\draw[arrow,#1] (#2) + (270:#3) arc(270:390:#3);
        % 4 arrow design.
        \draw[arrow,#1] (#2) + (55:#3) arc(55:145:#3);
        \draw[arrow,#1] (#2) + (145:#3) arc(145:235:#3);
        \draw[arrow,#1] (#2) + (235:#3) arc(235:325:#3);
        \draw[arrow,#1] (#2) + (325:#3) arc(325:415:#3);
    }

    % Flow + SE3
    \def\iteroutputs{
        \tikz{\node[embedding] {Mo-Emb};}\\
        %{\vspace{-0.38cm}}\\%extra vertical space between the two elements.
        \tikz{\node[se3_field] {SE(3)-Fld};}
    }

    \foreach \scale in {1,2,3,4}  {
        \pgfmathsetmacro{\xskip}{9 * \scale}
        \pgfmathsetmacro{\updateradius}{0.7}
        \pgfmathtruncatemacro{\resolution}{pow(2,5-\scale)}
        \pgfmathtruncatemacro{\bilinearupsample}{pow(2,4-\scale)}

        % Update loop
        \node[module,matching] (dense-se3-\scale) at (\xskip,0) {Dense-SE3};
        \node[red!60!black] (T-\scale) at ($(dense-se3-\scale.east) + (\updateradius,0)$) {$T_\scale$};
        \circledarrow{red!60!black}{T-\scale}{\updateradius};
        \coordinate (top-\scale) at ($(T-\scale)+(0,\updateradius)$);
        \node[module,matching,anchor=south] (update-\scale) at ($(T-\scale) + (0,\updateradius)$) {Update};
        \node[module,costvol,anchor=west] (costvolume-\scale) at ($(T-\scale) + (\updateradius,0)$) {Matching\\Costs};
        \node[container,anchor=north] (flow-\scale) at ($(T-\scale) + (0,-\updateradius)$) {};
        \node[se3_field, yshift=-0.4cm] (se3-1-\scale) at (flow-\scale.center) {SE(3)-Fld};
        \node[embedding, yshift=0.4cm] (embedding-1-\scale) at (flow-\scale.center) {Mo-Emb};

        % Inputs
        \node[module,encoder, xshift=0.25cm, yshift=0.35cm] (feature-\scale-1) at ({{0,2.1}} -| costvolume-\scale) {Features 1};
        \node[module,encoder,xshift=0.4cm] (feature-\scale-2) at ({{0,2.1}} -| costvolume-\scale) {Features 2};
        \node[module,encoder] (context-\scale)   at ({{0,2.1}} -| update-\scale) {Context};
        \node[module,encoder, xshift=-2.15cm, yshift=0.35cm] (depth1-\scale)   at ({{0,2.1}} -| update-\scale) {Depth 1};
        \node[module,encoder, xshift=-2.00cm] (depth2-\scale)   at ({{0,2.1}} -| update-\scale) {Depth 2};

        % Upsample + Loss
        \ifthenelse{\equal{\scale}{4}}{
            % Last scale has fewer upsampling steps.
            \node[upsample,supervision,yshift=-1.8cm] (upmask-\scale) at (flow-\scale) {$\Uparrow\!\times 2$};
            % \node[se3_field, yshift=-1.3cm] (upfinal-\scale) at (upmask-\scale) {SE(3)-Fld};
            \node[module,upsample_col, yshift=-1.1cm] (loss-\scale) at (upmask-\scale) {Loss};
        }{
            % Scale 1,2,3
            \node[upsample,supervision,xshift=4.2cm] (upmask-\scale) at (flow-\scale) {$\Uparrow\!\times 2$};
            \node[upsample,supervision, yshift=-1.8cm] (upbilinear-\scale) at (upmask-\scale) {$\uparrow\!\times\bilinearupsample$};
            % \node[se3_field, yshift=-1.3cm] (upfinal-\scale) at (upbilinear-\scale) {SE(3)-Fld};
            \node[module,upsample_col, yshift=-1.1cm] (loss-\scale) at (upbilinear-\scale) {Loss};
        }

        % For the first scale we have an extra node and bigger grouping.
        \ifthenelse{\equal{\scale}{1}}{
            % Initialization box.
            \node[module, flow, xshift=-2.7cm] (init) at (flow-\scale) {Initialization};
            %\node[module, flow, yshift=-1.6cm] (init) at (flow-\scale) {Init};% ADJUST dashed arrow between scales!
            \draw[arrow,dashed] (init) -- (flow-1);

            % Left scale area grouping. Includes init box. A bit wider because of the extra width due the init box.
            \node[
                fit=(costvolume-\scale)(update-\scale)(dense-se3-\scale)(flow-\scale)(top-\scale)(feature-\scale-1)(feature-\scale-2)(context-\scale)(depth1-\scale)(depth2-\scale)(init),
                label={[name=label-\scale,anchor=south,rotate=90]left:$\frac{1}{\resolution} \times (h,w)$},inner sep=0.1cm
            ] (scale-\scale) {};
            \begin{scope}[on background layer]
                \node[
                    thick,rounded corners,fill=gray!10!white,inner sep=0.1cm,
                    fit=(scale-\scale)(label-\scale)
                ] (scale-\scale) {};
            \end{scope}
        }{
            % Left scale area grouping
            \node[
                fit=(costvolume-\scale)(update-\scale)(dense-se3-\scale)(flow-\scale)(top-\scale)(feature-\scale-1)(feature-\scale-2)(context-\scale)(depth1-\scale)(depth2-\scale),
                label={[name=label-\scale,anchor=south,rotate=90]left:$\frac{1}{\resolution} \times (h,w)$},inner sep=0.1cm
            ] (scale-\scale) {};
            \begin{scope}[on background layer]
                \node[
                    thick,rounded corners,fill=gray!10!white,inner sep=0.1cm,
                    fit=(scale-\scale)(label-\scale)
                ] (scale-\scale) {};
            \end{scope}
        }

        % Arrows.
        % Feature arrows.
        \draw[arrow] (feature-\scale-2.south -| costvolume-\scale)  -- (costvolume-\scale);
        % Depth arrows.
        \draw[arrow] (depth2-\scale)  |- (update-\scale);
        % Other arrows.
        \draw[arrow] (context-\scale) -- (update-\scale);
        \draw[arrow] (flow-\scale) -- (upmask-\scale);
        \ifthenelse{\equal{\scale}{4}}{
            \draw[arrow] (upmask-\scale) -- (loss-\scale);

        }{
            % Scale 1,2,3
            \draw[arrow] (upmask-\scale) -- (upbilinear-\scale);
            \draw[arrow] (upbilinear-\scale) -- (loss-\scale);
        }
    }

    % Big right original resolution area grouping
    % Add invisible nodes for extra vertical space that matches areas on the left in height.
    %\node[module,opacity=0,draw, xshift=10cm] (top-node) at (costvolume-3) {Matching\\Costs};
    %\node[module,opacity=0,draw, xshift=10cm] (bottom-node) at (dense-se3-1) {Dense-SE3};
    \node[
        fit=(loss-1)(loss-2)(loss-3)(loss-4),%(top-node)(bottom-node),
        label={[name=label,anchor=south]below:$(h,w)$},
    ] (original-scale) {};
    \begin{scope}[on background layer]
        \node[
            thick,rounded corners,fill=gray!10!white,inner sep=0.1cm,
            fit=(original-scale)(label),
        ] (original-scale) {};
    \end{scope}

    % Dashed arrows between scales.
    \draw[arrow,dashed] (upmask-1) -- node[below] {Initialize} (flow-2);
    \draw[arrow,dashed] (upmask-2) -- node[below] {Initialize} (flow-3);
    \draw[arrow,dashed] (upmask-3) -- node[below] {Initialize} (flow-4);

\end{tikzpicture}
